TokenMotion: Decoupled Motion Control via Token Disentanglement for Human-centric Video Generation

Human-centric motion control in video generation remains a critical challenge, particularly when jointly controlling camera movements and human poses in scenarios like the iconic Grammy Glambot moment. While recent video diffusion models have made significant progress, existing approaches struggle with limited motion representations and inadequate integration of camera and human motion controls. In this work, we present TokenMotion, the first DiT-based video diffusion framework that enables fine-grained control over camera motion, human motion, and their joint interaction. We represent camera trajectories and human poses as spatio-temporal tokens to enable local control granularity. Our approach introduces a unified modeling framework utilizing a decouple-and-fuse strategy, bridged by a human-aware dynamic mask that effectively handles the spatially-and-temporally varying nature of combined motion signals. Through extensive experiments, we demonstrate TokenMotion's effectiveness across both text-to-video and image-to-video paradigms, consistently outperforming current state-of-the-art methods in human-centric motion control tasks. Our work represents a significant advancement in controllable video generation, with particular relevance for creative production applications.

==> experiments/Ablation/results.tex <==


% \begin{table}[htbp]
%   \centering
%     \begin{tabular}{cccccc}
%     \toprule
%     {\small Decouple} & {\small Hybrid} & {\small Token} & \multicolumn{3}{c}{} \\
%     {\small Fusion} & {\small Mask} & {\small Compression} & LPIPS$\downarrow$ & FID$\downarrow$ & FVD$\downarrow$ \\
%     \midrule
%     $\times$ & $\times$ & $\times$ & 0.57 & 88.11 & 402.34 \\
%     $\checkmark$ & $\times$ & $\times$ & 0.66 & 93.89 & 890.39 \\
%     $\times$ & $\checkmark$ & $\times$ & 0.54 & 88.56 & 590.62 \\
%     $\times$ & $\times$ & $\checkmark$ & 0.55 & 89.63 & \textbf{358.76} \\
%     $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{0.46} & \textbf{82.36} & 361.03 \\
%     \bottomrule
%     \end{tabular}%
%     \caption{Ablation studies with component breakdown. $\checkmark$ indicates the component is used, while $\times$ indicates it is not used.}
%   \label{tab:ablation}%
% \end{table}

==> experiments/Human-motion/qualitative1.tex <==
\begin{figure}[htbp]
    \centering
    \begin{tabular}{@{}ccc@{}}
        \begin{subfigure}{0.33\columnwidth}
            \centering
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s3Gg_f0.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s3Gg_f1.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s3Gg_f2.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s3Gg_f3.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s3Gg_f4.jpg}
            \caption{Person-object}
            \label{fig:multi people}
        \end{subfigure}
        \begin{subfigure}{0.33\columnwidth}
            \centering
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s2Gg_f0.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s2Gg_f1.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s2Gg_f2.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s2Gg_f3.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_0s2Gg_f4.jpg}
            \caption{Multi-Person}
            \label{fig:person with object}
        \end{subfigure}
        \begin{subfigure}{0.33\columnwidth}
            \centering
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_48hT9_f0.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_48hT9_f1.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_48hT9_f2.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_48hT9_f3.jpg} \\[-1pt]
            \includegraphics[width=\textwidth]{images/posecontrol/composition/sample_48hT9_f4.jpg}
            \caption{Combined}
            \label{fig:person with object}
        \end{subfigure}
    \end{tabular}
    \caption{Human-motion control with complex composition.}
    \label{fig:compositional human-motion control.}
\end{figure}

==> experiments/Human-motion/results.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
    \begin{tabular}{lcccc}
    \toprule
          & SSIM  & PSNR  & FID   & FVD \\
    \midrule
    MagicAnimate~\cite{MagicAnimate24Xu} &       &       &       &  \\
    AnimateAnyone~\cite{AnimateAnyone24Hu} &       &       &       &  \\
    Ours  &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \caption{Quantitative evaluation results for human-motion-only control video generation.}
  \label{tab:camera-only results}%
\end{table}%


==> experiments/Joint_Control_Results/main_results.tex <==
\begin{table*}[htbp]
    \footnotesize
    \centering
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{clccccccccccc}
    \toprule
    \toprule
          & \multirow{2}[4]{*}{Method} & \multicolumn{3}{c}{General Metrics} &       & \multicolumn{3}{c}{Camera Metrics} &       & \multicolumn{2}{c}{Human-Motion Metrics} &  \\
\cmidrule{3-5}\cmidrule{7-9}\cmidrule{11-12}          &       & LPIPS$\downarrow$ & FID$\downarrow$   & FVD$\downarrow$   &       & KptsErr$\downarrow$ & RotErr$\downarrow$ & TransErr$\downarrow$ &       & PoseErr$\downarrow$ & DetErr$\downarrow$ &  \\
    \midrule
    \multirow{5}[2]{*}{T2V} & MotionCtrl & 0.623 & 116.41 & 1185.83 &       & 6.72  & 0.47  & 8.66  &       & 172.44 & 14.73 &  \\
          & Direct-A-Video & 0.67  & 132.08 & 941.05 &       & \textbf{3.85}  & \textbf{0.24}  & \textbf{5.06}  &       & 173.26 & 10.68 &  \\
          & MotionBooth & 0.69  & 125.62 & 795.59 &       & 5.24  & 0.36  & 6.42  &       & 165.49 & 13.19 &  \\
          & CogVideoX\* & 0.57  & 88.11 & 402.34 &       &   -    &   -    &    -   &      &    -   &    -   &  \\
          & Ours  & \textbf{0.46} & \textbf{82.36} & \textbf{361.03} &       & 4.43  & 0.27  & 5.34  &       & \textbf{45.24} & \textbf{2.5} &  \\
    \midrule
    \multirow{2}[2]{*}{I2V} & ImageConductor & 0.43  & 131.36 & 878.59 &       & 4.32  & 0.44  & 5.44  &       & 164.28 & 9.18  &  \\
          & Ours  & \textbf{0.42} & \textbf{74.65} & \textbf{332.27} &       & \textbf{3.77} & \textbf{0.22} & \textbf{2.98} &       & \textbf{83.82} & \textbf{3.63} &  \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    
    \caption{Quantitative comparisons for joint controlling camera and human motion for both T2V and I2V generation. \* denotes the original CogVideoX model, whose camera metrics and human-motion metrics are not calculated because no motion control is performed.}
    \label{tab:main results}
\end{table*}




==> images/jointcontrol/prompts.tex <==
% case-1 prompt: Two women are walking hand in hand along a winding road during sunset with rolling hills, distant mountains, and a clear, golden sky.

% case-2 prompt: Two women are having a conversation in a lush, green field with overcast skies, one wearing a black and white checkered coat, black hat, and carrying a light pink handbag, while the other is in a beige coat and long, straight brown hair, and holding a smartphone.
